An orthogonal approach to the subfactor of a planar algebra

By changing to an orthogonal basis, we give a short proof that the subfactor of the graded algebra of a planar algebra reproduces the planar algebra.

==> tee <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 1500 3150 1500 3825
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 2400 3150 2400 3825
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 3300 3150 3300 3825
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 4200 3150 4200 3825
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 5100 3150 5100 3825
2 1 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 2
	 6000 3150 6000 3825
2 2 0 6 0 7 50 -1 -1 0.000 0 0 -1 0 0 5
	 825 1200 6825 1200 6825 3150 825 3150 825 1200
4 0 0 50 -1 0 30 0.0000 4 15 315 2400 2250    \001
4 0 0 50 -1 0 60 0.0000 4 630 540 2775 2400 T\001
4 0 0 50 -1 0 60 0.0000 4 405 435 3375 2850 n\001

